Understanding, Implementing, and Supporting Security Assurance Cases in Safety-Critical Domains

The increasing demand for connectivity in safety-critical domains has made security assurance a crucial consideration. In safety-critical industry, software, and connectivity have become integral to meeting market expectations. Regulatory bodies now require security assurance cases (SAC) to verify compliance, as demonstrated in ISO/SAE-21434 for automotive. However, existing approaches for creating SACs do not adequately address industry-specific constraints and requirements. In this thesis, we present CASCADE, an approach for creating SACs that aligns with ISO/SAE-21434 and integrates quality assurance measures. CASCADE is developed based on insights from industry needs and a systematic literature review. We explore various factors driving SAC adoption, both internal and external to companies in safety-critical domains, and identify gaps in the existing literature. Our approach addresses these gaps and focuses on asset-driven methodology and quality assurance. We provide an illustrative example and evaluate CASCADE's suitability and scalability in an automotive OEM. We evaluate the generalizability of CASCADE in the medical domain, highlighting its benefits and necessary adaptations. Furthermore, we support the creation and management of SACs by developing a machine-learning model to classify security-related requirements and investigating the management of security evidence. We identify deficiencies in evidence management practices and propose potential areas for automation. Finally, our work contributes to the advancement of security assurance practices and provides practical support for practitioners in creating and managing SACs.

==> TexFiles/Chapter1.tex <==
%Here you can just include the entire paper, starting from the first section.
%Skip all the meta Latex code, e.g., begin{document}, includes and so on.

\input{TexFiles/paperA/main}
%\input{TexFiles/paperA/02_conclusion}

==> TexFiles/Chapter1_abstract.tex <==
\newpage
\section*{Abstract}
Assurance cases are structured arguments that are commonly used to reason about the safety of a product or service. Currently, there is an ongoing push towards using assurance cases for also cybersecurity, especially in safety critical domains, like automotive. While the industry is faced with the challenge of defining a sound methodology to build security assurance cases, the state of the art is rather immature. Therefore, we have conducted a thorough investigation of the (external) constraints and (internal) needs that security assurance cases have to satisfy when used in the automotive industry. This has been done in the context of two large automotive companies. The end result is a set of recommendations that automotive companies can apply in order to define security assurance cases that are (i) aligned with the constraints imposed by the existing and upcoming standards and regulations and (ii) harmonized with the internal product development processes and organizational practices. We expect the results to be also of interest for product companies in other safety critical domains, like healthcare, transportation, and so on.\\ 
\linebreak
\textbf{Keywords: } security; assurance cases; automotive
\newpage
